Estimating 3D Motion and Forces of Person-Object Interactions from Monocular Video

In this paper, we introduce a method to automatically reconstruct the 3D motion of a person interacting with an object from a single RGB video. Our method estimates the 3D poses of the person and the object, contact positions, and forces and torques actuated by the human limbs. The main contributions of this work are three-fold. First, we introduce an approach to jointly estimate the motion and the actuation forces of the person on the manipulated object by modeling contacts and the dynamics of their interactions. This is cast as a large-scale trajectory optimization problem. Second, we develop a method to automatically recognize from the input video the position and timing of contacts between the person and the object or the ground, thereby significantly simplifying the complexity of the optimization. Third, we validate our approach on a recent MoCap dataset with ground truth contact forces and demonstrate its performance on a new dataset of Internet videos showing people manipulating a variety of tools in unconstrained environments.

==> eval_2Dpose_est.tex <==
\label{appendix:objectpose}
\section{Estimating 2D object pose.}

\paragraph{Evaluation metrics.}
%In addition to human 3D pose, we further show qualitative results of the estimated 3D object pose.
In addition to the human 3D pose, we evaluate also the accuracy of the estimated 2D object pose.
%The objects that we consider have small volume and are highly ambiguous due to rotational symmetry, making it difficult to apply the state-of-the-art 3D object estimators such as BB8~\cite{rad2017bb8}.
For quantitative evaluation, we calculate the 2D end-point reprojection error and proportion of detections, as well as the bounding box AP$_{50}$ (IoU threshold $0.5$). Reference 2D end-point locations were annotated manually using the VIA annotator \cite{dutta2016via} in 3 keyframes per video. The bounding boxes are defined as orthogonal \jiri{Josef: is this the correct adjective?} boxes with the end-points in opposite corners \jiri{Josef: This seems to be the most reasonable definition so that all bounding boxes are comparable}.

\paragraph{Results}

We compare the final estimate by trajectory optimization and the initial estimate by Mask R-CNN (see Table~\ref{tb:bboxerror}).
The results show that the human 3D pose contains surprisingly rich information to disambiguate the 2D pose for objects.% see below:
%Since the object appearance in the wrench and carjack videos is very weak, we only apply the ground plane constraints in these videos and show the advantage of modelling ground contact in the final results.

%I would do first the 2D keypoint reprojection errors as we have discussed as they are clearer. it is unclear how to deal with missing frames, i.e. what should be the error when a method does not predict an object in a frame and the other does. We should see how often this occurs. I am afraid it may occur a lot. We would like to penalize methods for not predicting.

\begin{table}[t]
\footnotesize
\centering
\caption{\small \textbf{2D object end-point localization results on the Handtool dataset.} For each tool we report the 2D end-point reprojection error (in pixels) / proportion of detections.}
\label{tb:endpointserror}
\begin{tabular}{lccccc}
\hline
\jiri{?} & Barbell & Scythe & Spade & Avg \\ \hline
Mask R-CNN & 44.3/0.77 & 24.4/0.87 & 23.9/0.83 & ... /0.82 \\
Ours & \textbf{.../1.0} & \textbf{...} & \textbf{...} & \textbf{...} \\ \hline
\end{tabular}
\end{table}

\begin{table}[t]
\footnotesize
\centering
\caption{\small \textbf{2D object end-point localization results on the Handtool dataset.} For each tool we report the bounding box AP$_{50}$. \jiri{Update Mask R-CNN numbers using just 5 videos selected by Zongmian.} \jiri{* denotes padding of 5 pixels, ** 10 pixels, *** 25 pixels}}
\label{tb:bboxerror}
\begin{tabular}{lcccccc}
\hline
AP$_{50}$ & Barbell & Hammer & Scythe & Spade & mAP$_{50}$ \\ \hline
Mask R-CNN* & $0.53$ & $0.6$ & $0.93$ & $0.8$ & $-$ \\
Ours*  & \textbf{$0.4$} & \textbf{$0.47$} & \textbf{$0.8$} & \textbf{$0.2$} & \textbf{$-$} \\ \hline
Mask R-CNN** & $0.6$ & $0.6$ & $0.93$ & $0.87$ & $-$ \\
Ours**  & \textbf{$0.47$} & \textbf{$0.47$} & \textbf{$0.8$} & \textbf{$0.27$} & \textbf{$-$} \\ \hline
Mask R-CNN** & $0.67$ & $0.6$ & $0.93$ & $0.93$ & $-$ \\
Ours**  & \textbf{$0.73$} & \textbf{$0.73$} & \textbf{$1.0$} & \textbf{$0.53$} & \textbf{$-$} \\ \hline
\end{tabular}
\end{table}

